BiRoDiff: Diffusion policies for bipedal robot locomotion on unseen terrains

Locomotion on unknown terrains is essential for bipedal robots to handle novel real-world challenges, thus expanding their utility in disaster response and exploration. In this work, we introduce a lightweight framework that learns a single walking controller that yields locomotion on multiple terrains. We have designed a real-time robot controller based on diffusion models, which not only captures multiple behaviours with different velocities in a single policy but also generalizes well for unseen terrains. Our controller learns with offline data, which is better than online learning in aspects like scalability, simplicity in training scheme etc. We have designed and implemented a diffusion model-based policy controller in simulation on our custom-made Bipedal Robot model named Stoch BiRo. We have demonstrated its generalization capability and high frequency control step generation relative to typical generative models, which require huge onboarding compute.

==> Reinforcement_Learning_Framework.tex <==
Our approach centers on sim-to-real reinforcement learning (RL) to cultivate bipedal locomotion skills, assuming a foundational understanding of RL \cite{sutton2018reinforcement}. In the broader RL framework, the robot's control policy $\pi$ operates discretely at each time step \(t\), taking in the current state \(s_t\) and producing an action \(a_t\). Executing this action leads to a transition to the subsequent state \(s_{t+1}\). The dynamics governing these state transitions remain unknown to the robot, influenced by environmental conditions such as terrain type and the inherent dynamics of the robot itself. As the learning process unfolds, each state transition corresponds to a real-valued reward \(r_t\), strategically aligned with predefined goals to incentivize desired behavior. Our RL optimization objective revolves around learning a policy that, through dynamic interaction with the environment, maximizes the expected cumulative discounted reward over a finite horizon \(T\). Formally, our goal is to discover a policy $\pi$ that maximizes the objective function: \(J(\pi) = \mathbb{E} \sum_{t=0}^{T} \gamma^t R_t\), where \(\gamma \in [0, 1]\) represents the discount factor, and \(R_t\) serves as a random variable denoting the reward at time \(t\) when following $\pi$ from a state drawn from an initial state distribution.


